Deep Clustering of Remote Sensing Scenes through Heterogeneous Transfer Learning

This paper proposes a method for unsupervised whole-image clustering of a target dataset of remote sensing scenes with no labels. The method consists of three main steps: (1) finetuning a pretrained deep neural network (DINOv2) on a labelled source remote sensing imagery dataset and using it to extract a feature vector from each image in the target dataset, (2) reducing the dimension of these deep features via manifold projection into a low-dimensional Euclidean space, and (3) clustering the embedded features using a Bayesian nonparametric technique to infer the number and membership of clusters simultaneously. The method takes advantage of heterogeneous transfer learning to cluster unseen data with different feature and label distributions. We demonstrate the performance of this approach outperforming state-of-the-art zero-shot classification methods on several remote sensing scene classification datasets.

==> figures/pipeline_fig_tikz.tex <==
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,261); %set diagram left start at 0, and has height of 261

%Shape: Square [id:dp822706218037031] 
\draw   (30,70) -- (100,70) -- (100,140) -- (30,140) -- cycle ;
%Shape: Square [id:dp12006188657082473] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=0.6 ] (40,60) -- (110,60) -- (110,130) -- (40,130) -- cycle ;
%Shape: Square [id:dp9876127383329176] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=0.35 ] (50,50) -- (120,50) -- (120,120) -- (50,120) -- cycle ;
%Shape: Rectangle [id:dp09335101115963185] 
\draw  [color={rgb, 255:red, 255; green, 1; blue, 1 }  ,draw opacity=1 ] (30,170) -- (80,170) -- (80,220) -- (30,220) -- cycle ;
%Shape: Rectangle [id:dp9580034719569466] 
\draw  [color={rgb, 255:red, 255; green, 1; blue, 1 }  ,draw opacity=0.6 ] (40,160) -- (90,160) -- (90,210) -- (40,210) -- cycle ;
%Shape: Rectangle [id:dp30251868798905823] 
\draw  [color={rgb, 255:red, 255; green, 1; blue, 1 }  ,draw opacity=0.35 ] (50,150) -- (100,150) -- (100,200) -- (50,200) -- cycle ;
%Rounded Rect [id:dp7862027965582543] 
\draw   (140,66) .. controls (140,57.16) and (147.16,50) .. (156,50) -- (204,50) .. controls (212.84,50) and (220,57.16) .. (220,66) -- (220,114) .. controls (220,122.84) and (212.84,130) .. (204,130) -- (156,130) .. controls (147.16,130) and (140,122.84) .. (140,114) -- cycle ;

%Rounded Rect [id:dp15518700639124816] 
\draw   (310,66) .. controls (310,57.16) and (317.16,50) .. (326,50) -- (374,50) .. controls (382.84,50) and (390,57.16) .. (390,66) -- (390,114) .. controls (390,122.84) and (382.84,130) .. (374,130) -- (326,130) .. controls (317.16,130) and (310,122.84) .. (310,114) -- cycle ;

%Rounded Rect [id:dp02070006201722374] 
\draw   (480,66) .. controls (480,57.16) and (487.16,50) .. (496,50) -- (544,50) .. controls (552.84,50) and (560,57.16) .. (560,66) -- (560,114) .. controls (560,122.84) and (552.84,130) .. (544,130) -- (496,130) .. controls (487.16,130) and (480,122.84) .. (480,114) -- cycle ;

%Shape: Rectangle [id:dp25577540377863595] 
\draw   (250,26.05) -- (274.47,26.05) -- (274.47,180) -- (250,180) -- cycle ;
%Shape: Rectangle [id:dp8959555227220377] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=0.6 ] (255.53,20) -- (280,20) -- (280,173.95) -- (255.53,173.95) -- cycle ;
%Shape: Rectangle [id:dp7199225558063236] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=0.35 ] (260,16.05) -- (284.47,16.05) -- (284.47,170) -- (260,170) -- cycle ;
%Shape: Rectangle [id:dp6016227772886582] 
\draw   (420,68.68) -- (444.47,68.68) -- (444.47,120) -- (420,120) -- cycle ;
%Shape: Rectangle [id:dp855266043522549] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=0.6 ] (425.53,64.34) -- (450,64.34) -- (450,115.66) -- (425.53,115.66) -- cycle ;
%Shape: Rectangle [id:dp4974381028032322] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=0.35 ] (430,60) -- (454.47,60) -- (454.47,111.32) -- (430,111.32) -- cycle ;
%Straight Lines [id:da0938798446835849] 
\draw    (110,90) -- (138,90) ;
\draw [shift={(140,90)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da84162529371598] 
\draw    (220,90) -- (248,90) ;
\draw [shift={(250,90)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da9581008617489479] 
\draw    (280,90) -- (308,90) ;
\draw [shift={(310,90)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da44795906992359646] 
\draw    (390,90) -- (418,90) ;
\draw [shift={(420,90)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da25534978998206537] 
\draw    (450,90) -- (478,90) ;
\draw [shift={(480,90)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Circle [id:dp4500087448357255] 
\draw   (600,35) .. controls (600,21.19) and (611.19,10) .. (625,10) .. controls (638.81,10) and (650,21.19) .. (650,35) .. controls (650,48.81) and (638.81,60) .. (625,60) .. controls (611.19,60) and (600,48.81) .. (600,35) -- cycle ;
%Shape: Circle [id:dp9558802592823517] 
\draw   (600,90) .. controls (600,76.19) and (611.19,65) .. (625,65) .. controls (638.81,65) and (650,76.19) .. (650,90) .. controls (650,103.81) and (638.81,115) .. (625,115) .. controls (611.19,115) and (600,103.81) .. (600,90) -- cycle ;
%Shape: Circle [id:dp42655341689109116] 
\draw   (600,175) .. controls (600,161.19) and (611.19,150) .. (625,150) .. controls (638.81,150) and (650,161.19) .. (650,175) .. controls (650,188.81) and (638.81,200) .. (625,200) .. controls (611.19,200) and (600,188.81) .. (600,175) -- cycle ;
%Straight Lines [id:da7083489038743771] 
\draw    (560,90) -- (598,90) ;
\draw [shift={(600,90)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da05384396312412365] 
\draw    (560,90) -- (598.82,36.62) ;
\draw [shift={(600,35)}, rotate = 126.03] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da18381602241497896] 
\draw    (560,90) -- (599.19,178.17) ;
\draw [shift={(600,180)}, rotate = 246.04] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Curve Lines [id:da4028594519660451] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ]   (90,190) .. controls (140.75,188.67) and (177.96,202.53) .. (179.97,131.08) ;
\draw [shift={(180,130)}, rotate = 91.31] [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (520,90) node   [align=left] {\begin{minipage}[lt]{45.22pt}\setlength\topsep{0pt}
\begin{center}
{\fontfamily{ptm}\selectfont Clustering}\\{\fontfamily{ptm}\selectfont Algorithm}
\end{center}

\end{minipage}};
% Text Node
\draw (350,90) node   [align=left] {\begin{minipage}[lt]{44.65pt}\setlength\topsep{0pt}
\begin{center}
{\fontfamily{ptm}\selectfont Manifold}\\{\fontfamily{ptm}\selectfont Projection}
\end{center}

\end{minipage}};
% Text Node
\draw (180,90) node   [align=left] {\begin{minipage}[lt]{40.67pt}\setlength\topsep{0pt}
\begin{center}
{\fontfamily{ptm}\selectfont Feature}\\{\fontfamily{ptm}\selectfont Extractor}
\end{center}

\end{minipage}};
% Text Node
\draw (625,130) node    {$\vdots $};
% Text Node
\draw (625,35) node    {$1$};
% Text Node
\draw (625,90) node    {$2$};
% Text Node
\draw (625,175) node    {$\hat{K}$};
% Text Node
\draw (20,2) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{84.75pt}\setlength\topsep{0pt}
\begin{center}
$\displaystyle n${\fontfamily{ptm}\selectfont  \ Inference Images}\\{\fontfamily{ptm}\selectfont (unlabeled)}
\end{center}

\end{minipage}};
% Text Node
\draw (81,212) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize] [align=left] {\begin{minipage}[lt]{78.93pt}\setlength\topsep{0pt}
\begin{center}
{\fontfamily{ptm}\selectfont Finetuning Images}\\{\fontfamily{ptm}\selectfont (labeled)}
\end{center}

\end{minipage}};
% Text Node
\draw (221,189) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{66.91pt}\setlength\topsep{0pt}
\begin{center}
$\displaystyle n\times d${\fontfamily{ptm}\selectfont  \ Features}
\end{center}

\end{minipage}};
% Text Node
\draw (386,139) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{66.91pt}\setlength\topsep{0pt}
\begin{center}
$\displaystyle n\times p${\fontfamily{ptm}\selectfont  \ Features}\\$\displaystyle p\ll d$
\end{center}

\end{minipage}};
% Text Node
\draw (553,202) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{86.88pt}\setlength\topsep{0pt}
\begin{center}
{\fontfamily{ptm}\selectfont Cluster Assignments}
\end{center}

\end{minipage}};


\end{tikzpicture}

